The Extractive-Abstractive Spectrum: Uncovering Verifiability Trade-offs in LLM Generations

Across all fields of academic study, experts cite their sources when sharing information. While large language models (LLMs) excel at synthesizing information, they do not provide reliable citation to sources, making it difficult to trace and verify the origins of the information they present. In contrast, search engines make sources readily accessible to users and place the burden of synthesizing information on the user. Through a survey, we find that users prefer search engines over LLMs for high-stakes queries, where concerns regarding information provenance outweigh the perceived utility of LLM responses. To examine the interplay between verifiability and utility of information-sharing tools, we introduce the extractive-abstractive spectrum, in which search engines and LLMs are extreme endpoints encapsulating multiple unexplored intermediate operating points. Search engines are extractive because they respond to queries with snippets of sources with links (citations) to the original webpages. LLMs are abstractive because they address queries with answers that synthesize and logically transform relevant information from training and in-context sources without reliable citation. We define five operating points that span the extractive-abstractive spectrum and conduct human evaluations on seven systems across four diverse query distributions that reflect real-world QA settings: web search, language simplification, multi-step reasoning, and medical advice. As outputs become more abstractive, we find that perceived utility improves by as much as 200%, while the proportion of properly cited sentences decreases by as much as 50% and users take up to 3 times as long to verify cited information. Our findings recommend distinct operating points for domain-specific LLM systems and our failure analysis informs approaches to high-utility LLM systems that empower users to verify information.

==> code_availability.tex <==
\section{Code Availability} 
\label{sec:code_availablity}

The code for implementing the evaluated systems, conducting MTurk evaluations with a custom web app interface, analyzing results, and generating the figures in the paper is available on GitHub.\footnote{\href{https://github.com/guestrin-lab/extractive-abstractive-spectrum}{https://github.com/guestrin-lab/extractive-abstractive-spectrum}} The software is distributed under the terms of the Apache License and can be accessed without restrictions.


==> data_availability.tex <==
\section{Data Availability} 
\label{sec:data_availablity}
The cited generations of the seven evaluated systems over four query distributions and the corresponding human evaluations are publicly available on Github.\footnote{\href{https://github.com/guestrin-lab/extractive-abstractive-spectrum}{https://github.com/guestrin-lab/extractive-abstractive-spectrum}} The user preference survey results are also available in the same repository. All data is anonymized, distributed under the terms of the Apache License, and can be accessed without restrictions.

==> ethics_and_inclusion.tex <==
% Has the research included local researchers throughout the research process – study design, study implementation, data ownership, intellectual property and authorship of publications?

% Is the research locally relevant and has this been determined in collaboration with local partners?

% Please describe whether roles and responsibilities were agreed amongst collaborators ahead of the research and whether any capacity-building plans for local researchers were discussed.

% Would this research have been severely restricted or prohibited in the setting of the researchers? If yes, please provide details on specific exceptions granted for this research in agreement with local stakeholders.

% Where appropriate, has the study been approved by a local ethics review committee? If not, please explain the reasons.

% Where animal welfare regulations, environmental protection and biorisk-related regulations in the local research setting were insufficient compared to the setting of the researchers, please describe if research was undertaken to the higher standards.

% Does the research result in stigmatization, incrimination, discrimination or otherwise personal risk to participants? If yes, describe provisions to ensure safety and well- being of participants.

% If research involves health, safety, security or other risk to researchers, describe any risk management plans undertaken.

% Have any benefit sharing measures been discussed in case biological materials, cultural artefacts or associated traditional knowledge has been transferred out of the country?

% Please indicate if you have taken local and regional research relevant to your study into account in citations.

Roles and responsibilities were agreed upon among collaborators before the research began. All authors were responsible for the design of experiments and interpretation of results. TW was solely responsible for the implementation of the experiments. Workers from the United States on the Prolific and Amazon Mechanical Turk platforms were compensated \$13.71/hour and \$16/hour for the user preference survey and cited generation evaluation, respectively, and had a direct line of communication with the authors. Collected data was anonymized. The authors declare no competing interests. 


==> output_examples/test.tex <==
\refstepcounter{egbox}
\begin{tcolorbox}[adjusted title=Example \theegbox, colback=white, arc=4mm, fontupper=\sffamily]
\raggedright
\noindent

\end{tcolorbox}


==> output_examples/utility_failure_info_retrieval.tex <==
% \refstepcounter{egbox}
% \begin{tcolorbox}[adjusted title=Example \theegbox, colback=white, arc=4mm, fontupper=\sffamily]
% \raggedright
% \noindent
% \textbf{NQ Query: }who produced a change is gonna come\vspace{.2cm}\\\textbf{Entailed Generation: }Insufficient information to generate a grounded response.\vspace{.2cm}\\\textbf{GPT-4 + Vertex Generation: }"A Change Is Gonna Come" was produced by Hugo \& Luigi, who were renowned record producers and songwriters, working alongside the song's writer and performer, Sam Cooke, in 1963.
% \end{tcolorbox}


\refstepcounter{egbox}
\begin{tcolorbox}[adjusted title=Example \theegbox, colback=white, arc=4mm, fontupper=\sffamily]
\raggedright
\noindent
\textbf{NQ Query: }who did cora marry in once upon a time\vspace{.2cm}\\\textbf{Quoted Generation: }Cora "seizes her moment at a masquerade ball, slyly sidling up to the eligible Prince Henry and charming him into asking her to dance" [1].\vspace{.2cm}\\\textbf{GPT-4 + Vertex Generation: }In "Once Upon a Time," Cora married Prince Henry, the father of Regina, also known as the Evil Queen. Their marriage was part of Cora's ambitious rise to power and royalty.\vspace{.2cm}\\\textbf{Gemini: }Cora married Prince Henry, who was the younger brother of King Leopold. Their union resulted in the birth of Regina, who would later become the Evil Queen.
\label{utility_failure_IR_failure}
\end{tcolorbox}


==> prompts/nq_abs_output_prompt.tex <==
\vspace{.2cm}
\begin{promptbox}
\raggedright
\textcolor{instructioncolor}{Instruction: }Respond to the following query by building off of the response below. Specifically, rephrase and combine the sentences in the response by paraphrasing them, cutting out extraneous or redundant information, and simplifying details that are too fine-grained with respect to the question. Also, simplify premises to their logical conclusions to more directly answer the query. Most importantly, use accurate outside information to make the revised response a more useful answer to the query. If the provided response is not an accurate or useful answer to the query, then extensively revise it with accurate outside information. Respond in no more than about 100 words. Do not refer to the response in your revised response.

\textcolor{querycolor}{Query:} What's the life cycle of a frog?

\textcolor{sourcescolor}{Response:} The stages of a frog’s life cycle are egg, larva, and adult. In a frog egg, the yolk splits into many cells which are the beginnings of a tadpole, or a frog larva. In one to three weeks, a small tadpole hatches from the egg. During the larval stage, tadpoles, or frogs’ larvae, are equipped with simple gills, a mouth, and a lengthy tail. As they develop, tadpoles consume plants and algae and then grow back legs, followed by front legs. Shortly afterward, their body begins to shift in shape and they gain the ability to consume insects. Then, the tails of the tadpoles grow smaller and skin develops over their gills while they grow eardrums and lungs.

\textcolor{responsecolor}{Revised Response: }A frog matures from egg, to tadpole, to adult in a process called metamorphosis. After hatching from an egg into a tadpole, it will grow back legs and then front legs, while storing nutrients in its long tail. As the tadpole loses its gills, it gains lungs. At this point, the tadpole is considered to be a froglet, until its tail shrinks away, at which point it is a frog.


\textcolor{instructioncolor}{Instruction: }Respond to the following query by building off of the response below. Specifically, rephrase and combine the sentences in the response by paraphrasing them, cutting out extraneous or redundant information, and simplifying details that are too fine-grained with respect to the question. Also, simplify premises to their logical conclusions to more directly answer the query. Most importantly, use accurate outside information to make the revised response a more useful answer to the query. If the provided response is not an accurate or useful answer to the query, then extensively revise it with accurate outside information. Respond in no more than about 100 words. Do not refer to the response in your revised response.

\textcolor{querycolor}{Query:} What are the benefits of hyaluronic acid for skin care?

\textcolor{sourcescolor}{Response:} Hyaluronic acid helps to retain moisture. It makes it easier for skin to be flexible and diminishes skin lines and wrinkles.

\textcolor{responsecolor}{Revised Response: }Hyaluronic acid helps keep skin moist and wrinkle-free. It can also reduce scarring, which may be especially beneficial for people who have had severe acne in the past.


\textcolor{instructioncolor}{Instruction: }Respond to the following query by building off of the response below. Specifically, rephrase and combine the sentences in the response by paraphrasing them, cutting out extraneous or redundant information, and simplifying details that are too fine-grained with respect to the question. Also, simplify premises to their logical conclusions to more directly answer the query. Most importantly, use accurate outside information to make the revised response a more useful answer to the query. If the provided response is not an accurate or useful answer to the query, then extensively revise it with accurate outside information. Respond in no more than about 100 words. Do not refer to the response in your revised response.

\textcolor{querycolor}{Query:} What is a heirloom tomato?

\textcolor{sourcescolor}{Response:} Unlike tomatoes that carry a genetic mutation that makes them look consistently red at the expense of their flavor, many heirloom tomatoes taste sweeter. Genuine heirloom tomatoes have to be old due to being a variety over the last 25 to 50 years.

\textcolor{responsecolor}{Revised Response: }Heirloom tomatoes are tomatoes that have a sweet flavor profile and are often other colors than red, including yellow, orange, and purple. A tomato variety is considered heirloom once it’s been a variety for 25-50 years, although some insist that at least 100 years is necessary.


\textcolor{instructioncolor}{Instruction: }Respond to the following query by building off of the response below. Specifically, rephrase and combine the sentences in the response by paraphrasing them, cutting out extraneous or redundant information, and simplifying details that are too fine-grained with respect to the question. Also, simplify premises to their logical conclusions to more directly answer the query. Most importantly, use accurate outside information to make the revised response a more useful answer to the query. If the provided response is not an accurate or useful answer to the query, then extensively revise it with accurate outside information. Respond in no more than about 100 words. Do not refer to the response in your revised response.

\textcolor{querycolor}{Query:} What's the flavor of juicy fruit gum?

\textcolor{sourcescolor}{Response:} the mixture of fruit flavors in Juicy Fruit is comprised of predominately lemon, orange, pineapple, and banana notes.

\textcolor{responsecolor}{Revised Response: }Juicy Fruit flavor is a blend of mostly orange, lemon, banana, and pineapple flavors. Some say it tastes like coconut and jackfruit as well.


\textcolor{instructioncolor}{Instruction: }Respond to the following query by building off of the response below. Specifically, rephrase and combine the sentences in the response by paraphrasing them, cutting out extraneous or redundant information, and simplifying details that are too fine-grained with respect to the question. Also, simplify premises to their logical conclusions to more directly answer the query. Most importantly, use accurate outside information to make the revised response a more useful answer to the query. If the provided response is not an accurate or useful answer to the query, then extensively revise it with accurate outside information. Respond in no more than about 100 words. Do not refer to the response in your revised response.

\textcolor{querycolor}{Query:} who invented the cornell method of note taking

\textcolor{sourcescolor}{Response:} The Cornell method of note-taking was invented in the 1950s by Walter Pauk, a professor of education at Cornell University.

\textcolor{responsecolor}{Revised Response: }\end{promptbox}
\refstepcounter{promptbox}
\textbf{Box \thepromptbox: } Example of the prompt with few-shot examples used to generate the abstractive output for NQ queries.
\label{box:nq_abs_output_prompt}
\vspace{.2cm}

==> prompts/nq_citation_prompt.tex <==
\vspace{.2cm}
\begin{promptbox}
\raggedright
\textcolor{instructioncolor}{Instruction: }Examine the text and numbered quotes below. The text was likely written from one or a few of the quotes. Which of these quotes, if any, could have been used to write the text? It may be none of the quotes, one quote, or several of the quotes. Do not provide redundant quotes. Respond with the number of the quote(s) in brackets.

\textcolor{querycolor}{Text:} As they develop, tadpoles consume plants and algae and then grow back legs, followed by front legs

\textcolor{sourcescolor}{Quotes:}

[1] "The life cycle of a frog consists of three stages: egg, larva, and adult"

[2] "As the frog grows, it moves through these stages in a process known as metamorphosis"

[3] "the yolk in each egg splits into more and more cells and begins to take the form of a tadpole, the larva of a frog"

[4] "Within one to three weeks, the egg is ready to hatch, and a tiny tadpole breaks free"

[5] "[t]adpoles, frogs' larvae, have rudimentary gills, a mouth, and a long tail"

[6] "tadpoles feed on algae and other vegetation"

[7] "they grow back legs, then front legs too"

[8] "Soon after, their body starts to change shape, and they’re able to start eating insects"

[9] "Next, the tadpoles’ tails shrink away, and skin grows over their gills, as they develop lungs and eardrums"

\textcolor{responsecolor}{Answer: }[6][7]


\textcolor{instructioncolor}{Instruction: }Examine the text and numbered quotes below. The text was likely written from one or a few of the quotes. Which of these quotes, if any, could have been used to write the text? It may be none of the quotes, one quote, or several of the quotes. Do not provide redundant quotes. Respond with the number of the quote(s) in brackets.

\textcolor{querycolor}{Text:} Hyaluronic acid has been shown to decrease the recovery time of wounds and can lessen scarring

\textcolor{sourcescolor}{Quotes:}

[1] "helps keep things hydrated"

[2] "helps skin stretch and flex and reduces skin wrinkles and lines"

[3] "Hyaluronic acid is also proven to help wounds heal faster and can reduce scarring"

\textcolor{responsecolor}{Answer: }[3]


\textcolor{instructioncolor}{Instruction: }Examine the text and numbered quotes below. The text was likely written from one or a few of the quotes. Which of these quotes, if any, could have been used to write the text? It may be none of the quotes, one quote, or several of the quotes. Do not provide redundant quotes. Respond with the number of the quote(s) in brackets.

\textcolor{querycolor}{Text:} Unlike tomatoes that carry a genetic mutation that makes them look consistently red at the expense of their flavor, many heirloom tomatoes taste sweeter

\textcolor{sourcescolor}{Quotes:}

[1] "Many heirloom tomatoes are sweeter and lack a genetic mutation that gives tomatoes a uniform red color at the cost of the fruit's taste"

[2] "True heirlooms must be 'old' because they have been a variety for anywhere between 25 and 50 years"

\textcolor{responsecolor}{Answer: }[1]


\textcolor{instructioncolor}{Instruction: }Examine the text and numbered quotes below. The text was likely written from one or a few of the quotes. Which of these quotes, if any, could have been used to write the text? It may be none of the quotes, one quote, or several of the quotes. Do not provide redundant quotes. Respond with the number of the quote(s) in brackets.

\textcolor{querycolor}{Text:} The Cornell note-taking system was developed in the 1950s by Walter Pauk, an education professor at Cornell University.

\textcolor{sourcescolor}{Quotes:}

[1] "was invented in the 1950s by Walter Pauk, a professor of education at Cornell University"

\textcolor{responsecolor}{Answer: }\end{promptbox}
\refstepcounter{promptbox}
\textbf{Box \thepromptbox: } Example of the prompt with few-shot examples used to identify the citations for the paraphrased, entailed, and abstractive responses to NQ queries.
\label{box:nq_citation_prompt}
\vspace{.2cm}

==> prompts/nq_ent_output_prompt.tex <==
\vspace{.2cm}
\begin{promptbox}
\raggedright
\textcolor{instructioncolor}{Instruction: }Respond to the following query by building off of the response below. Specifically, rephrase and combine the sentences in the response by paraphrasing them, cutting out extraneous or redundant information, and simplifying details that are too fine-grained with respect to the question. Also, simplify premises to their logical conclusions to more directly answer the query. Do not refer to the response in your revised response.

\textcolor{querycolor}{Query:} What's the life cycle of a frog?

\textcolor{sourcescolor}{Response:} The stages of a frog’s life cycle are egg, larva, and adult. Growing through these stages is a process called metamorphosis. In a frog egg, the yolk splits into many cells which are the beginnings of a tadpole, or a frog larva. In one to three weeks, a small tadpole hatches from the egg. During the larval stage, tadpoles, or frogs’ larvae, are equipped with simple gills, a mouth, and a lengthy tail. As they develop, tadpoles consume plants and algae and then grow back legs, followed by front legs. Shortly afterward, their body begins to shift in shape and they gain the ability to consume insects. Then, the tails of the tadpoles grow smaller and skin develops over their gills while they grow eardrums and lungs.

\textcolor{responsecolor}{Revised Response: }The stages of a frog’s life cycle are egg, larva, and adult. Growing through these stages is a process called metamorphosis. Cells in the yolk of a frog egg form a tadpole, or a frog larva. In one to three weeks, a small tadpole hatches from the egg. During the larval stage, tadpoles are equipped with simple gills, a mouth, and a lengthy tail. As they develop, tadpoles consume plants and algae and then grow back legs, followed by front legs. Shortly afterward, they gain the ability to consume insects. Then, the tails of the tadpoles shrink, they lose their gills, and they grow eardrums and lungs.


\textcolor{instructioncolor}{Instruction: }Respond to the following query by building off of the response below. Specifically, rephrase and combine the sentences in the response by paraphrasing them, cutting out extraneous or redundant information, and simplifying details that are too fine-grained with respect to the question. Also, simplify premises to their logical conclusions to more directly answer the query. Do not refer to the response in your revised response.

\textcolor{querycolor}{Query:} What are the benefits of hyaluronic acid for skin care?

\textcolor{sourcescolor}{Response:} Hyaluronic acid helps to retain moisture. It makes it easier for skin to be flexible and diminishes skin lines and wrinkles. Hyaluronic acid has been shown to decrease the recovery time of wounds and can lessen scarring.

\textcolor{responsecolor}{Revised Response: }Hyaluronic acid helps to retain moisture. It makes it easier for skin to be flexible and diminishes wrinkles. Hyaluronic acid may decrease the recovery time of wounds and can lessen scarring.


\textcolor{instructioncolor}{Instruction: }Respond to the following query by building off of the response below. Specifically, rephrase and combine the sentences in the response by paraphrasing them, cutting out extraneous or redundant information, and simplifying details that are too fine-grained with respect to the question. Also, simplify premises to their logical conclusions to more directly answer the query. Do not refer to the response in your revised response.

\textcolor{querycolor}{Query:} What is a heirloom tomato?

\textcolor{sourcescolor}{Response:} Unlike tomatoes that carry a genetic mutation that makes them look consistently red at the expense of their flavor, many heirloom tomatoes taste sweeter. Genuine heirloom tomatoes have to be old due to being a variety over the last 25 to 50 years.

\textcolor{responsecolor}{Revised Response: }Unlike tomatoes that carry a genetic mutation that makes them look consistently red at the expense of their flavor, many heirloom tomatoes taste sweeter. Genuine heirloom tomatoes have been a variety over the last 25 to 50 years.


\textcolor{instructioncolor}{Instruction: }Respond to the following query by building off of the response below. Specifically, rephrase and combine the sentences in the response by paraphrasing them, cutting out extraneous or redundant information, and simplifying details that are too fine-grained with respect to the question. Also, simplify premises to their logical conclusions to more directly answer the query. Do not refer to the response in your revised response.

\textcolor{querycolor}{Query:} What's the flavor of juicy fruit gum?

\textcolor{sourcescolor}{Response:} the mixture of fruit flavors in Juicy Fruit is comprised of predominately lemon, orange, pineapple, and banana notes.

\textcolor{responsecolor}{Revised Response: }Juicy Fruit flavor is a blend of mostly orange, lemon, banana, and pineapple flavors.


\textcolor{instructioncolor}{Instruction: }Respond to the following query by building off of the response below. Specifically, rephrase and combine the sentences in the response by paraphrasing them, cutting out extraneous or redundant information, and simplifying details that are too fine-grained with respect to the question. Also, simplify premises to their logical conclusions to more directly answer the query. Do not refer to the response in your revised response.

\textcolor{querycolor}{Query:} who invented the cornell method of note taking

\textcolor{sourcescolor}{Response:} The Cornell method of note-taking was invented in the 1950s by Walter Pauk, a professor of education at Cornell University.

\textcolor{responsecolor}{Revised Response: }\end{promptbox}
\refstepcounter{promptbox}
\textbf{Box \thepromptbox: } Example of the prompt with few-shot examples used to generate the entailed output for NQ queries.
\label{box:nq_ent_output_prompt}
\vspace{.2cm}

==> prompts/nq_pp_output_prompt.tex <==
\vspace{.2cm}
\begin{promptbox}
\raggedright
\textcolor{instructioncolor}{Instruction: }Respond to the following query by building off of the response below. Specifically, rephrase each sentence in the response using a more fluent and useful wording to convey the same information. In other words, paraphrase each sentence of the response as an improved new sentence, with respect to the query. Do not refer to the response in your revised response.

\textcolor{querycolor}{Query:} What's the life cycle of a frog?

\textcolor{sourcescolor}{Response:} The life cycle of a frog consists of three stages: egg, larva, and adult. As the frog grows, it moves through these stages in a process known as metamorphosis. During the egg stage, the yolk in each egg splits into more and more cells and begins to take the form of a tadpole, the larva of a frog. Within one to three weeks, the egg is ready to hatch, and a tiny tadpole breaks free. In the larval stage, [t]adpoles, frogs' larvae, have rudimentary gills, a mouth, and a long tail. As they grow, tadpoles feed on algae and other vegetation, and eventually, they grow back legs, then front legs too! Soon after, their body starts to change shape, and they’re able to start eating insects. Next, the tadpoles’ tails shrink away, and skin grows over their gills, as they develop lungs and eardrums!

\textcolor{responsecolor}{Paraphrased Response: }The stages of a frog’s life cycle are egg, larva, and adult. Growing through these stages is a process called metamorphosis. In a frog egg, the yolk splits into many cells which are the beginnings of a tadpole, or a frog larva. In one to three weeks, a small tadpole hatches from the egg. During the larval stage, tadpoles, or frogs’ larvae, are equipped with simple gills, a mouth, and a lengthy tail. As they develop, tadpoles consume plants and algae and then grow back legs, followed by front legs. Shortly afterward, their body begins to shift in shape and they gain the ability to consume insects. Then, the tails of the tadpoles grow smaller and skin develops over their gills while they grow eardrums and lungs.


\textcolor{instructioncolor}{Instruction: }Respond to the following query by building off of the response below. Specifically, rephrase each sentence in the response using a more fluent and useful wording to convey the same information. In other words, paraphrase each sentence of the response as an improved new sentence, with respect to the query. Do not refer to the response in your revised response.

\textcolor{querycolor}{Query:} What are the benefits of hyaluronic acid for skin care?

\textcolor{sourcescolor}{Response:} Hyaluronic acid helps keep things hydrated. It helps skin stretch and flex and reduces skin wrinkles and lines. Hyaluronic acid is also proven to help wounds heal faster and can reduce scarring.

\textcolor{responsecolor}{Paraphrased Response: }Hyaluronic acid helps to retain moisture. It makes it easier for skin to be flexible and diminishes skin lines and wrinkles. Hyaluronic acid has been shown to decrease the recovery time of wounds and can lessen scarring.


\textcolor{instructioncolor}{Instruction: }Respond to the following query by building off of the response below. Specifically, rephrase each sentence in the response using a more fluent and useful wording to convey the same information. In other words, paraphrase each sentence of the response as an improved new sentence, with respect to the query. Do not refer to the response in your revised response.

\textcolor{querycolor}{Query:} What is a heirloom tomato?

\textcolor{sourcescolor}{Response:} Many heirloom tomatoes are sweeter and lack a genetic mutation that gives tomatoes a uniform red color at the cost of the fruit's taste. True heirlooms must be 'old' because they have been a variety for anywhere between 25 and 50 years.

\textcolor{responsecolor}{Paraphrased Response: }Unlike tomatoes that carry a genetic mutation that makes them look consistently red at the expense of their flavor, many heirloom tomatoes taste sweeter. Genuine heirloom tomatoes have to be old due to being a variety over the last 25 to 50 years.


\textcolor{instructioncolor}{Instruction: }Respond to the following query by building off of the response below. Specifically, rephrase each sentence in the response using a more fluent and useful wording to convey the same information. In other words, paraphrase each sentence of the response as an improved new sentence, with respect to the query. Do not refer to the response in your revised response.

\textcolor{querycolor}{Query:} What's the flavor of juicy fruit gum?

\textcolor{sourcescolor}{Response:} the mixture of fruit flavors in Juicy Fruit is comprised of predominately lemon, orange, pineapple, and banana notes. 

\textcolor{responsecolor}{Paraphrased Response: }Juicy Fruit flavor is a blend of mostly orange, lemon, banana, and pineapple flavors.


\textcolor{instructioncolor}{Instruction: }Respond to the following query by building off of the response below. Specifically, rephrase each sentence in the response using a more fluent and useful wording to convey the same information. In other words, paraphrase each sentence of the response as an improved new sentence, with respect to the query. Do not refer to the response in your revised response.

\textcolor{querycolor}{Query:} who invented the cornell method of note taking

\textcolor{sourcescolor}{Response:} The Cornell method of note-taking was invented in the 1950s by Walter Pauk, a professor of education at Cornell University.

\textcolor{responsecolor}{Paraphrased Response: }\end{promptbox}
\refstepcounter{promptbox}
\textbf{Box \thepromptbox: } Example of the prompt with few-shot examples used to generate the paraphrased output for NQ queries.
\label{box:nq_pp_output_prompt}
\vspace{.2cm}


==> prompts/test.tex <==
\vspace{.2cm}
\begin{promptbox}

\textcolor{instructioncolor}{Instruction: }Respond to the following query by building off of the response below. Specifically, rephrase and combine the sentences in the response by paraphrasing them, cutting out extraneous or redundant information, and simplifying details that are too fine-grained with respect to the question. Also, simplify premises to their logical conclusions to more directly answer the query. Most importantly, use accurate outside information to make the revised response a more useful answer to the query. If the provided response is not an accurate or useful answer to the query, then extensively revise it with accurate outside information. Respond in no more than about 100 words. Do not refer to the response in your revised response.

\textcolor{querycolor}{Query:} What can you do to prevent migraine with brainstem aura?

\textcolor{sourcescolor}{Response:} To prevent migraine with brainstem aura, it helps to avoid the things that usually cause one. This includes being sure to Get enough sleep, Limit your stress, and Exercise daily. Additionally, Eat a balanced diet, Avoid drugs and alcohol, Don't skip meals,  and Limit caffeine. Avoid any foods that have been triggers.

\textcolor{responsecolor}{Revised Response: }Preventing migraine with brainstem aura involves lifestyle adjustments and possibly medication for those with frequent episodes. Key strategies include maintaining regular sleep patterns, managing stress, exercising regularly, eating a balanced diet, avoiding known food triggers, limiting caffeine and alcohol intake, and not skipping meals. Furthermore, If you don't respond to other treatments and you have 4 or more migraine days a month, your doctor may suggest preventive medicines, including seizure medicines, blood pressure medicines (like beta blockers and calcium channel blockers), and some antidepressants. Also, CGRP inhibitors are a new class of preventive medicine. There is anecdotal evidence that triptans can worsen migraine symptoms, even though it is often prescribed by medical professionals.


\textcolor{instructioncolor}{Instruction: }Respond to the following query by building off of the response below. Specifically, rephrase and combine the sentences in the response by paraphrasing them, cutting out extraneous or redundant information, and simplifying details that are too fine-grained with respect to the question. Also, simplify premises to their logical conclusions to more directly answer the query. Most importantly, use accurate outside information to make the revised response a more useful answer to the query. If the provided response is not an accurate or useful answer to the query, then extensively revise it with accurate outside information. Respond in no more than about 100 words. Do not refer to the response in your revised response.

\textcolor{querycolor}{Query:} What should I do if my child has a biting injury?

\textcolor{sourcescolor}{Response:} The first thing to do for any biting injury is to wash the area with soap and water. Even little teeth can break the skin. If the bite is bleeding and the wound appears to be deep, call your child's doctor. The bite may need medical treatment, which could include antibiotics or a tetanus shot, or both.

\textcolor{responsecolor}{Revised Response: }For a biting injury, immediately clean the wound with soap and water. If it's bleeding or deep, contact your child's doctor for potential treatment, which may involve antibiotics or a tetanus shot. If the child was bitten by an animal, it can be life-saving to seek medical treatment for a rabies vaccine within 24 hours, or at least within 72 hours. Even if more than 72 hours have elapsed since the bite, it is still not too late to get the shot. If left untreated, rabies can be fatal.


\textcolor{instructioncolor}{Instruction: }Respond to the following query by building off of the response below. Specifically, rephrase and combine the sentences in the response by paraphrasing them, cutting out extraneous or redundant information, and simplifying details that are too fine-grained with respect to the question. Also, simplify premises to their logical conclusions to more directly answer the query. Most importantly, use accurate outside information to make the revised response a more useful answer to the query. If the provided response is not an accurate or useful answer to the query, then extensively revise it with accurate outside information. Respond in no more than about 100 words. Do not refer to the response in your revised response.

\textcolor{querycolor}{Query:} Can I give cough and cold medicines to children under 4?

\textcolor{sourcescolor}{Response:} Talk to your pediatrician before giving OTC cold and cough medicines. These medicines should not be given to children under 4 years of age, according to the FDA and the drug makers.

\textcolor{responsecolor}{Revised Response: }The FDA and drug makers advise against giving cough and cold medicines to children under 4. Also, never give adult medicines to children; only use medicines designed for children. Lastly, do not give aspirin to a child due to the risk of Reye's syndrome, which is a rare but serious condition.


\textcolor{instructioncolor}{Instruction: }Respond to the following query by building off of the response below. Specifically, rephrase and combine the sentences in the response by paraphrasing them, cutting out extraneous or redundant information, and simplifying details that are too fine-grained with respect to the question. Also, simplify premises to their logical conclusions to more directly answer the query. Most importantly, use accurate outside information to make the revised response a more useful answer to the query. If the provided response is not an accurate or useful answer to the query, then extensively revise it with accurate outside information. Respond in no more than about 100 words. Do not refer to the response in your revised response.

\textcolor{querycolor}{Query:} How do I treat a blister?

\textcolor{sourcescolor}{Response:} Most blisters caused by friction or minor burns do not require a doctor's care. New skin will form underneath the affected area and the fluid is simply absorbed. Do not puncture a blister unless it is large, painful, or likely to be further irritated. The fluid-filled blister keeps the underlying skin clean, which prevents infection and promotes healing. But if you need to pop a blister or it pops by itself: Use a sterilized needle (to sterilize it, put the point or edge in a flame until it is red hot, or rinse it in alcohol). Wash your hands and the area thoroughly, then make a small hole; the fluid will drain on its own. If the fluid is white or yellow, the blister may be infected and needs medical attention. Do not remove the skin over a broken blister. The new skin underneath needs this protective cover. Apply an antibiotic ointment or cream. Look for signs of infection to develop, including pus drainage, red or warm skin surrounding the blister, or red streaks leading away from the blister.

\textcolor{responsecolor}{Revised Response: }For most blisters, medical care isn't necessary. Allow new skin to form beneath the blister and the fluid to absorb. To protect the blister from further irritation, it is advisable to cover it with moleskin, a durable cotton fabric with an adhesive backing available at most drug stores. If a blister is large, painful, or might be further irritated, and needs to be popped, sterilize a needle with heat or alcohol, clean your hands and the blister area, then gently puncture it to let the fluid drain, but don't remove the overlying skin as it protects the new skin. If the blister's fluid isn't clear (indicating possible infection), seek medical attention. Apply an antibiotic ointment, cover it with a bandage and monitor for signs of infection like pus, redness, or warmth.


\textcolor{instructioncolor}{Instruction: }Respond to the following query by building off of the response below. Specifically, rephrase and combine the sentences in the response by paraphrasing them, cutting out extraneous or redundant information, and simplifying details that are too fine-grained with respect to the question. Also, simplify premises to their logical conclusions to more directly answer the query. Most importantly, use accurate outside information to make the revised response a more useful answer to the query. If the provided response is not an accurate or useful answer to the query, then extensively revise it with accurate outside information. Respond in no more than about 100 words. Do not refer to the response in your revised response.

\textcolor{querycolor}{Query:} What medications can I use to lessen my child's teething pain?

\textcolor{sourcescolor}{Response:} Use baby acetaminophen (Tylenol) to dull pain. Do not use ibuprofen unless the baby is at least 6 months old.

\textcolor{responsecolor}{Revised Response: }\end{promptbox}
\refstepcounter{promptbox}
\textbf{Box \thepromptbox: } Example of the prompt with few-shot examples used to generate the abstractive output for MASH queries.
\label{box:mash_abs_output_prompt}
\vspace{.2cm}
